A Visual Cooperative Localization Method for Airborne Magnetic Surveying Based on a Manifold Sensor Fusion Algorithm Using Lie Groups

Recent advancements in UAV technology have spurred interest in developing multi-UAV aerial surveying systems for use in confined environments where GNSS signals are blocked or jammed. This paper focuses airborne magnetic surveying scenarios. To obtain clean magnetic measurements reflecting the Earth's magnetic field, the magnetic sensor must be isolated from other electronic devices, creating a significant localization challenge. We propose a visual cooperative localization solution. The solution incorporates a visual processing module and an improved manifold-based sensor fusion algorithm, delivering reliable and accurate positioning information. Real flight experiments validate the approach, demonstrating single-axis centimeter-level accuracy and decimeter-level overall 3D positioning accuracy.

==> sections/fiducial/detection.tex <==
The section presents the experimental results on own collected data.  The evaluation results on public datasets are given in~\cref{sec:add_exp_res_fid}.
\subsection{Classification Results On the Test Dataset }
Here we show some images that are misclassified by the classifier in~\cref{fig:cnn_images}. Please refer to~\cref{sec:fid_det_recog} for the information related to the classifier and the test dataset. As can be seen, some images may have been mislabeled, particularly the images in which the fiducial is partially occluded or incomplete. It is arguable whether those images should be labeled as \textit{Other} or \textit{Candidate}. Nonetheless, we could see that in most of the misclassified images, the fiducial is either occluded, partly out of view, or extremely tilted. Hence, even if they could be correctly classified, they may not provide correct positioning information. Considering the results shown in~\cref{fig:conf}, we could conclude that the overall performance of the classifier is satisfactory.
Future work will consider making the training dataset and test dataset more complete by relabeling those fuzzy images.

\begin{figure}[!ht]
    \centering
    \begin{minipage}[b]{.495\linewidth}
    \centering{
    \includegraphics[width=1\linewidth]{figures/fiducial/label_noobj_predict_obj_new.png}}
    \centering{\vspace{-1em}(a)}
    \end{minipage}
    \begin{minipage}[b]{.495\linewidth}
    \includegraphics[width=1\linewidth]{figures/fiducial/label_obj_predict_noobj_new.png}
    \centering{\vspace{-1em}(b)} 
    \end{minipage}
    \caption[Visual results of some misclassified images]{Visual results of some misclassified images. (a): List of images labeled as \textit{Other} but classified as \textit{Candidate}. (b): List of images labeled as \textit{Candidate} but classified as \textit{Other}.}
    \label{fig:cnn_images}
\end{figure}

\subsection{Evaluation Results of Tracking on Collected Datasets}
\label{sec:tracking_exp}
To thoroughly evaluate the trackers' performance in our use case, we collected three real flight datasets in 2019 at the DTU campus. 
In each dataset, there is a raw video sequence (around 2 to 2.5 minutes) captured by the GoPro camera.
%in which there are two fiducials.
% In the evaluation, we use template matching to initialize a tracker for one fiducial. 
In the evaluation, we use template matching to initialize one fiducial as the target, which is later tracked by the selected visual trackers. After initialization, template matching will no longer be performed, even if a tracker fails to follow the object. 
% We report the time when the first tracking failure happens.
We report the first tracking failure time for each tracker.
Since all trackers are initialized simultaneously, this time can be used as a measure to assess the endurance and robustness of a tracker.
% to fast motion and blur. 
Additionally, the FPS is also reported as a measure of efficiency. 
Quantitative results are listed in~\cref{tb:visual_tracking_own}.
One surprising observation is that DAT, although performs not well on the VTB dataset (see~\cref{sec:add_detection_tracking}), works very well on the collected datasets. Besides this exception, all the other observations remain the same, e.g., KCF is still the fastest tracker, while ECOHC is the most powerful tracker, but the slowest. 
\begin{table}[!ht]
	\centering
	\caption{{Evaluation results of concerned visual trackers on collected datasets.}}
	\begin{tabular}{c|c|c|c|c}
		\hline
		& \multicolumn{3}{c}{\textbf{Failure time: (s)}}  & \textbf{Mean FPS} \\ \cline{2-5}
        \textbf{Sequence Number} & 1 & 2 & 3 &   \\ \cline{1-4}
		\textbf{Total time of the seq} &  112.4 & 180 & 103.2 &  \\ \hline
		\textbf{ECOHC} & 112.4 & 145.7 &  103.2 &  49.9 \\ \hline
		\textbf{fDSST} & 70.7 & 78.9 & 103.2 &  186.8 \\ \hline
		\textbf{CACF} & 70.5 & 78.9 & 103.2 &  296.1 \\ \hline
		\textbf{Staple} & 112.4 & 78.9 & 103.2 &  81.9 \\ \hline
		\textbf{KCF} & 70.5 & 78.9 & 103.2 &  \cellcolor{yellow!20} 623.6 \\ \hline
		\textbf{DAT} & 112.4 & \cellcolor{yellow!20}152.7 & 103.2 &  134.7 \\ \hline
		\hline
	\end{tabular}
	\label{tb:visual_tracking_own}
\end{table}

~\cref{fig:tracking_fails} lists some representative images, on which some trackers fail to follow the target. As can be seen, tracking failures are primarily due to fast motion and image blur. More visual results can be reviewed in associated videos\footnote{\url{https://doi.org/10.5281/zenodo.4457136}}.
\begin{figure}[!ht]
    \centering
    \includegraphics[width=0.49\linewidth]{figures/fiducial/002109.png}
    \includegraphics[width=0.49\linewidth]{figures/fiducial/002667.png}\\
    \includegraphics[width=0.49\linewidth]{figures/fiducial/004658.png}
    \includegraphics[width=0.49\linewidth]{figures/fiducial/004883.png}\\
    \caption[Some representative images on which trackers fail to follow the target.]{Some representative images on which trackers fail to follow the target. The primary reasons for tracking failure are fast motion and blur. }
    \label{fig:tracking_fails}
\end{figure}

\subsection{Evaluation Results of the Visual Preprocessing Module on Collected Datasets}
\label{sec:Preprocessing_exp}
Here we present the evaluation results of the visual preprocessing module on the collected datasets mentioned above. 
\cref{fig:prepro_snap} shows two representative pictures of the ROIs detected by the visual processing module. 
The left image shows the performance when the thick rope occludes fiducials. 
The right image demonstrates the visual processing module's performance when fiducials are tilted due to the fast motion.
As can be seen, the visual processing module can detect ROIs correctly in both cases. 
To give a quantitative analysis, the success rate is reported in~\cref{tb:prepro_snap_tb}. 
Visual results can be found in the associated videos \footnote{\url{https://doi.org/10.5281/zenodo.4457136}}.

\begin{figure}[!ht]
    \centering
    \includegraphics[width=1\linewidth]{figures/fiducial/preprocessing_snap.png}
    \caption{Two representative pictures of the ROIs detected by the visual processing module. The detected ROIs are represented using light-blue and light orange bounding boxes.}
    \label{fig:prepro_snap}
\end{figure}
\begin{figure}[!ht]
    \centering
    \includegraphics[width=0.5\linewidth]{figures/fiducial/outofview.png}
    \caption{Failure case: the fiducials are out of view of the GoPro camera.}
    \label{fig:prepro_outofview}
\end{figure}
\begin{table}[!h]
	\centering
	\caption{{Quantitative evaluation results of the visual preprocessing module on collected datasets}}
	\begin{tabular}{c|c|c|c}
		\hline \hline
		& \multicolumn{3}{c}{\textbf{Sequence Number}} \\ \cline{2-4}
         & 1 & 2 & 3   \\ \cline{2-4}
		\textbf{Success Rate} & $100\%$ & $98.0\%$ &  $100\%$  \\ \hline
		\hline
	\end{tabular}
	\label{tb:prepro_snap_tb}
\end{table}
Overall speaking, the preprocessing module performs very well, being able to detect ROIs correctly in almost all the cases encountered. In only a few cases, it cannot detect the ROI properly. Apart from the aforementioned cases, including fast motion and blur, another failure case is when the fiducials are not within the view of the camera, as shown in~\cref{fig:prepro_outofview}. However, we argue this is not an important factor since if the camera cannot see the fiducials, it is impossible for the preprocessing module to detect them. 

\section{Evaluation Results of the Ellipse Detection Module}
\label{sec:res_ellp}
\begin{table}[!h]
	\centering
	\caption{{Quantitative evaluation results of the ellipse detection module on collected datasets}}
	\begin{tabular}{c|c|c|c}
		\hline
		& \multicolumn{3}{c}{\textbf{Sequence Number}} \\ \cline{2-4}
         & 1 & 2 & 3   \\ \cline{2-4}
		\textbf{Success Rate} & $98.8\%$ & $94.4\%$ &  $99.6\%$  \\ \hline
		\hline
	\end{tabular}
	\label{tb:ellip_detec_rb}
\end{table}
The performance of the ellipse detection module has been tested on the collected datasets mentioned above. Similarly, we list the success rate for each dataset in~\cref{tb:ellip_detec_rb}. Some representative visual results are shown in~\cref{fig:vs_own_1,fig:vs_own_3}. As can be seen, the developed arc-based ellipse detector can handle the occlusion caused by the rope very well. Moreover, when the view angle is extremely tilted, the detector also demonstrated good performance, although we witnessed a few false detections. 
The reason for yielding those false detections is explained as follows. As the two markers are close to each other, if the cropped patch contains two markers or one marker plus large portions from another marker, arcs from different markers may be grouped to determine an ellipse. Possible solutions include: 
\begin{itemize}
    \item Enhance the preprocessing module so that it can produce more precise ROIs.
    \item Physically enlarge the distance between the two markers.
    \item Use an additional positional constraint in the ellipse detector so that arcs distant from each other will not be grouped together.
\end{itemize}

\newpage
\begin{figure}[H]
    \centering
    \includegraphics[width=1\linewidth]{figures/fiducial/Slide7_new.PNG}
    \caption[Representative visual results of ellipse detection on collected datasets: partial occlusion.]{Representative visual results of ellipse detection on collected datasets. The black arrow indicates the time flow. This figure highlights the performance under partial occlusion.}
    \label{fig:vs_own_1}
\end{figure}
\begin{figure}[H]
    \centering
    \includegraphics[width=1\linewidth]{figures/fiducial/Slide8_new.PNG}
    \caption[Representative visual results of ellipse detection on collected datasets: tilted view angle.]{Representative visual results of ellipse detection on collected datasets. The black arrow indicates the time flow. This figure highlights the performance when the view angle is extremely tilted.}
    \label{fig:vs_own_3}
\end{figure}

==> sections/fiducial/fiducial.tex <==
\cref{fig:fd_ellip_detect} shows the detailed scheme chart of the ellipse detection module. It contains five steps. First arcs are extracted from the input image, and then related arcs are grouped together. Next,  ellipse fitting is applied to estimate ellipses. Once an ellipse is fitted, it is used to prune the arcs that also lie on the fitted ellipse. 
Fitted ellipses are clustered to suppress duplicate detections. Finally, validation is applied to filter out false detections. Each step will be described in detail below.
\begin{figure}[!ht]
    \centering
    \includegraphics[width=1.0\linewidth]{figures/fiducial/ellipse_detection.png}
    \caption[Scheme chart of the ellipse detection module.]{Scheme chart of the ellipse detection module.}
    \label{fig:fd_ellip_detect}
\end{figure}
\subsubsection{Arc Extraction}
Basically, there are two commonly used representations of arcs in the literature:
\begin{itemize}
    \item An arc is represented by a contour~\cite{fornaciari2014fast,jia2017fast}.
    \item An arc is represented by a list of connected line segments~\cite{puatruaucean2012parameterless,prasad2012edge,lu2019arc,meng2020arc}.
\end{itemize}
% Depending on how an arc is characterized, 
If the scene texture is very complex, the first representation may be problematic as background pixels would corrupt real arcs by adding diverged branches, see~\cref{fig:arc_contour} for an example. By contrast, the second representation is more reliable, in particular, if the line segments are detected by a robust detector~\cite{von2012lsd} that has false control capability. Hence, we also choose the second representation. 
\begin{figure}[!ht]
    \centering
    \includegraphics[width=0.4\linewidth]{figures/fiducial/arc_contour_res.png}
    \caption[Results of arc contour detection.]{Results of arc contour detection: yellow arrows point out the places where the detected arc contours contain undesired diverged branches due to the cluttered background texture. Contours in different quadrants are shown with different colors. We highlight the arcs with dashed ellipses that are corrupted by background pixels.}
    \label{fig:arc_contour}
\end{figure}
To detect LS, we use the detector (in short, LSD) proposed by~\cite{von2012lsd}, which is an efficient and robust line segment detector. 
Since straight LSs are unlikely to stem from arcs, they can be pruned without further processing. 
To distinguish straight LSs with non-straight LSs, we employ the PCA to compute the ratio between the largest eigenvalue and the smallest eigenvalue, which can be used as an indicator of straightness. 
A simulation is conducted to illustrate the main idea and validate its feasibility. In the simulation, we generate an arc with an increasing radius (from 30 pixels to 1000 pixels) in a $100\times100$ image. Since a line segment can be approximated by an arc from a circle whose radius is infinitely large, with the increasing of the radius, the arc generated will be more and more close to a line segment. 
We then use image morphological operations (more specifically, first dilation and then erosion) to make the arc bold. Points of the arc are extracted and fed to PCA. Suppose the eigenvalues of the resulting covariance matrix are $\lambda_1,\lambda_2$, and $\lambda_1>\lambda_2$, we compute the indicator as $\frac{\lambda_1}{\lambda_2}$. The result is shown in~\cref{fig:pca_lsd}. Clearly, the more straight the arc is, the larger the ratio will be. Therefore, with this indicator's help, the straight LSs can be pruned while other LSs are left for further processing. More importantly, for two reasons, computing this indicator will not improve the computational complexity. 
First, as the covariance matrix is a $2\times2$ matrix, its eigenvalues can be solved analytically.
Second, the covariance matrix has already been computed in the LSD for retrieving the line segment direction. Hence, we do not need to compute it again. An example of LSs detection is shown in~\cref{fig:ls_lsd}.
\begin{figure}[!ht]
    \centering
    \includegraphics[width=0.4\linewidth]{figures/fiducial/pca-full.png}
    \caption[Illustration of using a PCA based indicator to evaluate the straightness of a line segment]{Illustration of using a PCA based indicator to evaluate the straightness of a line segment: a batch of images are generated with arcs from curved to straight. PCA is conducted for each image and the ratio between the largest eigenvalue and the smallest eigenvalue is analyzed. Clearly, with the increase of the radius (i.e. the increase of the straightness), the ratio will also grow.}
    \label{fig:pca_lsd}
\end{figure}

\begin{figure}[!ht]
    \centering
    \includegraphics[width=1\linewidth]{figures/fiducial/lsd_res_s.png}
    \caption[Results of line segment detection.]{Results of line segment detection: figures, from left to right, are the raw image, the image with all LSs, the image with the LSs after pruning the straight LSs, the image with extracted arcs.}
    \label{fig:ls_lsd}
\end{figure}

\begin{figure}[!ht]
    \centering
    \includegraphics[width=0.8\linewidth]{figures/fiducial/linking.png}
    \caption[Illustration of linking LSs to form arcs.]{Illustration of linking LSs to form arcs. Drawing elements: grid indicates the neighborhood, small arrows denote the line segment direction, lines in light red are not considered as candidate LSs since their included angles are beyond the threshold. Identified arcs are enclosed with dashed envelopes.}
    \label{fig:linking}
\end{figure}
After non-straight LSs are extracted, they could be linked to form arcs. Separate LSs are linked based on a proximity and curvature constraint to ensure smoothness. The exact operations are described as follows and visually illustrated in~\cref{fig:linking}. 
For each LS (query LS), we search in the neighborhood of its start point and endpoint for candidate LSs to link. The size of the neighborhood controls the proximity. If a candidate LS exists in the neighborhood, the included angle between the query LS and the candidate LS is computed. If the included angle is smaller than a threshold, the candidate LS could be linked to the query LS. If there are more than one candidates that can be linked to the query LS, multiple arcs will be generated with each of them corresponds to one candidate LS. By recursively searching using the head and tail LS of an arc (using the first-in-first-out queue), the arc would link all possible LSs. 
The last figure in~\cref{fig:ls_lsd} shows the result of arc extraction.

\begin{figure}
    \centering
    \includegraphics[width=0.35\linewidth]{figures/fiducial/span.png}
    \caption[Illustration of span angle estimation.]{Illustration of span angle estimation. Assuming two points on an ellipse are $\mb{p}_1$ and $\mb{p}_2$, the ellipse center will lie on the line (dashed line) passing their midpoint $\mb{m}_1$ and intersection point $\mb{q}_1$ of their tangents (dotted line). Therefore, it is possible to estimate the ellipse center $\mb{c}$ using three points and their gradients. Once the center $\mb{c}$ is obtained, the span angle can be easily computed.}
    \label{fig:span}
\end{figure}
Finally, for each retrieved arcs, its span angle can be roughly estimated using the geometric relationship noted by~\cite{yuen1989detecting}. The basic idea is illustrated in~\cref{fig:span}. Taking two points and their gradients, the midpoints ($\mb{m}_1$ and $\mb{m}_2$) and the intersection points ($\mb{q}_1$ and $\mb{q}_2$) of their tangents can be found. The ellipse center geometrically lies on the line passing the midpoint and the intersection point. Therefore, the ellipse center can be estimated from three points and their gradients. Then the span angle of the arc can be easily computed. Here, the start point, the endpoint, and the COM of an arc are used as the three points. 
Although the estimated center may not be very accurate due to the noise~\cite{fornaciari2014fast}, it suffices to provide a rough estimation of the span angle used later to rank arcs.

\begin{figure}
    \centering
    \includegraphics[width=0.5\linewidth]{figures/fiducial/convexity.png}
    \caption[Illustration of region constraint used for arc grouping.]{Illustration of region constraint used for arc grouping. The Arc in black is the query arc. In this example, arc 1 is the query arc. Arc 1 can be grouped with arc 2 and arc 3, but not arc 4 and arc 5 as they are not in the proper region (shaded area). Arc 6 is in the region, but arc 1 is not in the proper region formed by arc 6. Therefore, arc 6 cannot be grouped with arc 1.}
    \label{fig:convexity}
\end{figure}
\subsubsection{Grouping}
As shown in~\ref{fig:algebraicfitting}, fitting with incomplete data (i.e., small arcs) will result in very bad estimates. Therefore, associating arcs that may belong to the same ellipse is of importance. 
Different grouping strategies have been proposed~\cite{fornaciari2014fast,prasad2012edge,meng2020arc,lu2019arc,jia2017fast}. However, most of those strategies are rule-based, which involves tuning quite a few parameters to achieve good performance. The strategy based on region analysis~\cite{prasad2012edge,meng2020arc,lu2019arc} stands out from those strategies thanks to its clear geometric meaning, which is used here for arc grouping.
As shown in~\cref{fig:convexity}, arc 1 can be grouped with arc 2 and arc 3, but not arc 4 and arc 5 as they are not in the proper region (shaded area). Mathematically, this requires us to check the dot products of the corresponding vectors, which can be written as follows
\begin{equation}
    \mb{n}_1\mb{v}_1 \geq 0,\ \mb{n}_1\mb{v}_2 \geq 0,\ \mb{n}_2\mb{v}_3 \geq 0,\ \mb{n}_2\mb{v}_4 \geq 0
\end{equation}
where $\mb{v}_i$ denotes a vector composed by the initial point of one arc to the initial point or the endpoint of another arc, and $\mb{n}_i$ denotes a normal vector of a LS. The one-way check cannot rule out one exception case, e.g., the arc 6 shown in~\cref{fig:convexity}. However, by mutually check the region constraint, the exception can be ruled out. It is worth noting that this constraint only serves as a necessary condition. In other words, arcs fulfilling this constraint are not guaranteed to be from the same ellipse. 

Instead of grouping arcs in an arbitrary order, we first rank arcs according to their span angle and then start grouping with the arc with the maximum span angle. Whenever a group is established, we will check the sum of the span angles. If the total span angle is over a threshold, ellipse fitting will immediately apply to this arc group. After fitting and a fast validation, the ellipse will be used to prune (described in~\cref{sec:on-the-fly-prune}) other arcs that fail to be associated with this arc group but still lie on the same ellipse. This iterative grouping-fitting-pruning technique will further reduce the number of trials needed to find out all ellipses. 

\subsubsection{Ellipse Fitting}
\label{sec:on-the-fly-prune}
Ellipse Fitting has been studied substantially in the literature. We review two classical approaches for ellipse fitting in~\cref{sec:ellipsefitting}. Briefly speaking, algebraic fitting is more efficient, while geometric fitting is more robust. Considering that there may be many combinations of different arcs waiting for ellipse fitting, we certainly need to prioritize efficiency. On these grounds, the direct method~\cite{fitzgibbon1999direct} is used for fast ellipse fitting. 

Even if the direct method is very efficient, it is still very time consuming if we attempt to fit exhaustively on different combinations of arcs. 
Luckily, there is a feasible acceleration which was first noticed by~\cite{wang2014fast} and later applied by~\cite{lu2019arc,meng2020arc}\footnote{Although both ~\cite{lu2019arc} and~\cite{meng2020arc} claimed they proposed the acceleration, we argue that the original contribution should be owed to the work by~\cite{wang2014fast}}. The underlying idea of this acceleration is straightforward. From~\cref{eq:ellip_fit_matrix}, it can be seen that the direct method needs to compute the scatter matrix $\mb{A}^\top\mb{A}$. By expanding it, we will have
\begin{equation}
\mb{A}^\top\mb{A}=\boldsymbol{\alpha}_1^\top\boldsymbol{\alpha}_1 + \cdots + \boldsymbol{\alpha}_n^\top\boldsymbol{\alpha}_n=\sum_{i=1}^{n} \boldsymbol{\alpha}_i^\top\boldsymbol{\alpha}_i
\label{eq:ellip_sum}
\end{equation}
where the definition of $\boldsymbol{\alpha}_i, i=1,\cdots,n$ is given in~\cref{eq:alpha_defi}. An interesting point revealed by~\cref{eq:ellip_sum} is that the scatter matrix $\mb{A}^\top\mb{A}$ is a summation of separate terms like $\boldsymbol{\alpha}_i^\top\boldsymbol{\alpha}_i$. Therefore, a similar technique to the integral chain can be used to incrementally compute the scatter matrix $\mb{A}^\top\mb{A}$. More specially, assuming a scatter matrix $\mb{A}^\top\mb{A}$ have been computed from a batch of points ($\mb{p}_i, i=1,\cdots,n$ ) and a few additional points ($\mb{p}_j, j = n+1, \cdots, n+k$) are found, a new scatter matrix $\mb{A}_{\text{new}}^\top\mb{A}_{\text{new}}$ for ellipse fitting, that jointly considers the batch of points and the new points, can be computed as follows:
$$
\mb{A}_{\text{new}}^\top\mb{A}_{\text{new}}=\sum_{i=1}^{n+k} \boldsymbol{\alpha}_i^\top\boldsymbol{\alpha}_i=\mb{A}^\top\mb{A} + \sum_{i=n+1}^{n+k} \boldsymbol{\alpha}_i^\top\boldsymbol{\alpha}_i
$$
As can be seen, the new scatter matrix does not need to be computed from scratch but can be ``integrated'' from previously computed scatter matrices. Based on this acceleration, it is feasible to compute the scatter matrix for each arc group merely once and then sum these matrices accordingly when ellipse fitting is applied. As reported in~\cite{wang2014fast,lu2019arc,meng2020arc}, the technique can dramatically reduce the computation time.

After an ellipse is fitted, a fast validation is performed by checking the number of inlier pixels. More specifically, for pixels inside the circumscribed rectangle of the LSs, their corresponding normal directions to the ellipse are computed and compared to their image gradient directions. If the gradient direction of a pixel is consistent with its normal direction (i.e., the angle difference is within a threshold), it is classified as an inlier point. After counting all inliers, the ratio between the number of inliers and the total length of the arcs in this group is computed and used as an indicator for fast validation. 

\begin{figure}
    \centering
    \includegraphics[width=0.8\linewidth]{figures/fiducial/prune.png}
    \caption{ Ellipse candidates detected without (left) and with (right) on-the-fly pruning. }
    \label{fig:on-the-flypruning}
\end{figure}

\paragraph{On-the-fly Pruning}
The on-the-fly pruning is used to further prune arcs that lie on the same ellipse but have not been added into the arc group used for fitting. 
Considering that the ellipse obtained from algebraic fitting on incomplete data is not very reliable, the prune is applied only when a salient ellipse is detected. 
The salience is evaluated by the total span angle of the arcs used for ellipse fitting. 
Instead of using the aforementioned roughly estimated span angle, we re-compute the span angle using the fitted ellipse center. 
If the span angle is over a threshold (e.g., $135^\circ$), the fitted ellipse is identified as a salient detection. 
The obtained ellipse parameters are then applied to each arc that is not in the fitting group to compute its mean algebraic distance to the estimated ellipse. 
If one arc has a mean algebraic distance lower than a criterion, it is added to the group and pruned from the list of arcs waiting for grouping. A new ellipse will be fitted after pruning if there are new arcs added to the fitting group. An example result is shown in~\cref{fig:on-the-flypruning}. As can be seen, pruning will trim out some invalid candidates, which can improve the efficiency.

\subsubsection{Clustering}
To prune duplicate detections, a clustering post-processing step is applied. In this step, an ellipse is represented with its parametric form, see~\cref{sec:ellipsefitting}, which means an ellipse can be treated as a five-dimensional point. However, this five-dimensional space is not a vector space due to the orientation angle.~\cite{lu2019arc} developed a hierarchical method by clustering on divided space: first on the ellipse centers (2D space), next on the orientations (1D space), and finally on the semi-major and semi-minor axes (2D space). However, this is not very efficient under our considerations. Instead, we suggest clustering first on a 4D space (i.e., the ellipse center,  the semi-major, and semi-minor axes) and then on a 1D space (i.e., the orientations). Similar to~\cite{lu2019arc}, the mean shift algorithm~\cite{cheng1995mean} is used for clustering.  As the mean shift algorithm requires repetitively query the nearest neighbor and neighbors within a window, we use a KDTree to accelerate the querying procedure.  Specifically, the KDTree is used when clustering on the 4D space. As the 4 parameters form a 4D vector space, we use the L2 distance as the metric to build the KDTree. Practically, the nanoflann library\footnote{Nanoflann: \url{https://github.com/jlblancoc/nanoflann}} is used in our implementation for building the KDTree.

\begin{figure}
    \centering
    \includegraphics[width=0.6\linewidth]{figures/fiducial/span_angle2.png}
    \caption[Illustration of angular coverage computation.]{Illustration of angular coverage computation. First, a histogram is established by voting from inlier points of a candidate ellipse. After voting, the interval with the longest contiguous nonzero bins is used as the angular coverage.}
    \label{fig:span_final}
\end{figure}
\begin{figure}
    \centering
    \includegraphics[width=0.6\linewidth]{figures/fiducial/final.png}
    \caption{Final ellipse detection results. This figure shows ellipses detected after clustering and validation.}
    \label{fig:ell_final}
\end{figure}
\subsubsection{Validation}
After proceeding with the aforementioned steps, we obtain a batch of possible ellipses from an input image. Before output, they have to be validated for their correctness. Validation is often based on some geometric indicators. The most often used indicators are the ratio of the number of support inliers on an ellipse to the perimeter of the ellipse~\cite{lu2019arc,jia2017fast} and the measure of angular coverage~\cite{meng2020arc,prasad2012edge,wang2014fast}, which are also used in this work. Since the ellipse perimeter does not have a closed-form solution, the following approximation is used~\cite{borwein1989ramanujan}:
\begin{equation}
L \approx \pi[3(a+b)-\sqrt{(3 a+b)(a+3 b)}]
\end{equation}
where $a$ and $b$ are the length of the semi-major axis and semi-minor axis, respectively. 
Further, a pixel is identified as an inlier if the Rosin distance~\cite{rosin1996analysing} from this pixel to an ellipse is lower than a distance threshold (e.g., 1 pixel) and its normal direction to the ellipse is consistent with its gradient direction. Concerning the angular coverage, we use the method suggested by~\cite{lu2019arc}. It first establishes a histogram, with each bin being an angular coverage interval. Each inlier pixel will then vote to this histogram using its angular position with respect to the semi-major axis. After voting, the interval with the longest contiguous nonzero bins is used as the angular coverage, as illustrated in~\cref{fig:span_final}. Assuming there are $N_\text{inlier}$ inliers for a candidate ellipse and the angular coverage is $\tau_s$, the indicator is computed as 
\begin{equation}
\mathbb{I}(\boldsymbol{\theta}_i) = \frac{N_\text{inlier}}{L} \mathbb{I}(\tau_s, \tau), \text{ where } \mathbb{I}(\tau_s, \tau)=\left\{
\begin{array}{c}
    1, \text{ if $\tau_s\geq \tau$}\\
    0, \text{ otherwise} 
\end{array}
\right.
\end{equation}
where $\boldsymbol{\theta}_i$ is the parametric parameters of the $i-th$ ellipse, and $\tau$ is a threshold of the angular coverage.~\cref{fig:ell_final} shows the final detected ellipses after clustering and validation.



\subsubsection{Final Output: Conic Matrix}
For each ellipse after validation, its conic matrix is computed, which will be used for positioning. Since the ellipse was detected from the local patch instead of the raw image, its conic matrix was computed with respect to the patch's local coordinate system. Before using it for positioning,  it has to be transformed to a corresponding conic matrix relative to the original image, which can be done as follows. We can consider the points on the local patches are obtained from their corresponding points on the original image after a translation. Therefore, let $\mathbf{u}_2=[x_2, y_2, 1]^\top$ be a point on the local patch and $\mathbf{u}_1=[x_1, y_1, 1]^\top$ the corresponding point on the original image, their relationship can be established by a pre-conditioning matrix $\mb{T}$ as
$$
\mathbf{u}_2 = \mb{T}\mathbf{u}_1,\quad \text{where } \mb{T}=\left[
\begin{array}{ccc}
    1 &  0 & -\Delta_x \\
    0 & 1 & -\Delta_y \\
    0 & 0 & 1
\end{array}
\right]
$$
where $\Delta_x, \Delta_y$ are the offsets that make $x_2 = x_1-\Delta_x,y_2 = y_1-\Delta_y$. According to \cref{eq:h_conic}, the corresponding conic matrix $\mb{C}_2$ on the original image can be computed from the conic matrix $\mb{C}_1$ on the local patch by
\begin{equation}
    \mb{C}_2 = \mb{T}^\top \mb{C}_1 \mb{T}
\end{equation}
The conic matrix $\mb{C}_2$ is the final output of the fiducial detection module and will be used in~\cref{sec:chapter6} for positioning.



==> sections/fiducial/processing.tex <==
An overview of the scheme chart of the preprocessing module is shown in~\cref{fig:fd_preprocessing}.
Initially, we extract ROI candidates using template matching and feed them into a CNN based classifier to recognize the correct candidates and reject others. The detected ROIs will be used by the ellipse detection module. In addition, they are also fed back to the preprocessing module to launch tracking. In the case of tracking failures, we switch back to detection to process the new image. 
\subsubsection{Candidate Extraction}
Template matching is employed for extracting candidate ROIs thanks to its efficiency. By sliding the templates across the whole image and computing a response at each anchor point, template matching creates a response map for the input image. To enhance the robustness to scale variations, an image pyramid is established, and the response map is computed at each layer of the pyramid. The final response map is a weighted combination of the response map from each layer. Since the scale variation is not very significant in our case, a two-layer image pyramid is sufficient. % computes a response map. 
The normalized square difference is chosen as the score to measure the coherence, which is defined as 
\begin{equation}
\text { score }(x, y)=\frac{\sum_{x^{\prime}, y^{\prime}}\left(T\left(x^{\prime}, y^{\prime}\right)-I\left(x+x^{\prime}, y+y^{\prime}\right)\right)^{2}}{\sqrt{\sum_{x^{\prime}, y^{\prime}} T\left(x^{\prime}, y^{\prime}\right)^{2} \cdot \sum_{x^{\prime} \cdot y^{\prime}} I\left(x+x^{\prime}, y+y^{\prime}\right)^{2}}}
\end{equation}
where $(x,y)$ denotes the anchor position where the score is computed, $(x^\prime,y^\prime)$ denotes the local coordinate of each pixel in the template, $T$ and $I$ represent the template and the search image, respectively. 
The target objects can be detected by searching the local minimum on the response map. 
A non-maximal suppression technique is applied to suppress duplicate responses and extract the best $K$ ($K=3$) responses, as illustrated in~\cref{fig:temp_match}. The template matching method's average timing is approximately 25 ms on an image of 676×380 pixels, or equivalently, 40 Hz.
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/fiducial/temp_match.png}
    \caption[Illustration of candidate extraction using template matching.]{Illustration of candidate extraction using template matching: figures, from left to right, are input downsampled image, response map computed by applying template matching, detected candidates using non-maximum suppression.}
    \label{fig:temp_match}
\end{figure}

\subsubsection{Recognition}
\label{sec:fid_det_recog}
Inevitably, the extracted ROIs may contain some false positives due to either noises or long term occlusion. Therefore, we verify the correctness of the proposed ROIs using a learning-based classifier. A CNN is applied for this task because CNNs have been shown superior performance over traditional machine learning methods that use handcraft features~\cite{goodfellow2016deep}. Considering the efficiency of the template matching submodule, we tend to use a lightweight and fast CNN for recognition.
\begin{figure}
    \centering
    \includegraphics[width=0.5\linewidth]{figures/fiducial/tinycnn}
    \caption{Illustration of the network structure of the designed CNN for recognition.}
    \label{fig:cnn}
\end{figure}
The structure of the designed CNN is depicted in~\cref{fig:cnn}. We use three convolutional (marked as conv) layers as the encoder for feature extraction and two fully connected layers (marked as fc) plus a softmax output layer for classification. The ReLU is used as the activation function and followed by a batch normalization.
This network was trained on a laptop with an Intel i7 2.8 GHz CPU and one Nvidia Quadro M2200 GPU. The standard stochastic gradient descent optimizer was used to train the network based on a labeled training dataset containing approximately 40000 images ($80\%$ for training, while the rest $20\%$ for validation). We test the trained network on a testing dataset that includes around 35000 images. The final testing accuracy is $99.39\%$, and the inference time is around 1.6 ms. The confusion matrix is shown in~\cref{fig:conf} and some representattive misclassified images are shown in~\cref{fig:cnn_images}.
\begin{figure}[!ht]
    \centering
    \includegraphics[width=0.5\linewidth]{figures/fiducial/cnn_conf3.png}
    \caption[Confusion matrix of the classifier.]{Confusion matrix of the classifier: the light green shaded cells correspond to correctly classified observations, while the light red shaded cells indicate incorrectly classified observations. The rightmost column lists the precision and the recall is shown at the bottom row. The last diagonal cell (the bottom-right cell) shows the overall accuracy.}
    \label{fig:conf}
\end{figure}

\subsubsection{Tracking}
\label{sec:detection_tracking}
As we expect the tracking algorithm to be faster than template matching and recognition (about 40 Hz), after surveying the performances of various trackers on different benchmarks~\cite{wu2013online,VOT_TPAMI}, our primary interest focuses on four correlation filter-based visual trackers~\cite{mueller2017context,henriques2014high,danelljan2016discriminative,danelljan2017eco} and two color-based trackers~\cite{bertinetto2016staple,possegger2015defense}, as summarized in~\cref{tb:tracker_summary}.
The theories concerning the correlation filters have been detailed clearly in two pioneering work~\cite{bolme2010visual,henriques2014high}. Therefore, we omit the theories and recommend interested readers refer to their work~\cite{bolme2010visual,henriques2014high} to obtain more information about the theory and derivation.

\begin{table}
	\centering
	\caption{{Summary of related visual trackers}}
	\begin{tabular}{c|c|c}
		\hline
		\textbf{Abbreviation } & \textbf{Type} & \textbf{Publication} \\ \hline
		ECOHC & Correlation Filter-Based & \cite{danelljan2017eco} \\ \hline
		fDSST & Correlation Filter-Based & \cite{danelljan2016discriminative} \\ \hline
		CACF & Correlation Filter-Based & \cite{mueller2017context} \\ \hline
		KCF & Correlation Filter-Based & \cite{henriques2014high} \\ \hline
		Staple & Color-based & \cite{bertinetto2016staple} \\ \hline
		DAT & Color-based & \cite{possegger2015defense} \\ \hline
	\end{tabular}
	\label{tb:tracker_summary}
\end{table}

To evaluate the selected trackers' real performance, experiments on the public benchmark proposed by~\cite{wu2013online} and own collected datasets were conducted, and the results can be found in~\cref{sec:add_detection_tracking} and in~\cref{sec:tracking_exp}, respectively. From the experimental results, we could conclude that: 
\begin{itemize}
    \item If precision and robustness are the priorities, choose ECOHC.
    \item If efficiency is the primary factor to be considered, KCF is the best choice.
\end{itemize}
All the selected tracking approaches may inevitably fail in practice. 
Therefore, identifying tracking failure timely is important to prevent the tracker from drifting away from the target.  
As suggested by~\cite{bolme2010visual}, the Peak-to-Sidelobe ratio,  which measures the strength of a correlation peak, can be used as a score for detecting tracking failure. However, empirically, we find that it is not very reliable to identify tracking failure by merely relying on this score. Hence, we use a ``strong'' threshold to alert potential tracking failures. In this context, strong means a threshold higher than the nominal value, which serves as a sufficient but not necessary condition.  
In case that tracking failure is detected,  the classifier is used to verify the validity of the tracked ROIs. Template matching is relaunched if the verification fails, which prevents the tracker from drifting away unconsciously.

\subsection{Combined System}
The developed preprocessing module is a combination of the three submodules mentioned above, which runs at 40-90 FPS on images of 676×380 pixels.
This speed is achieved on a laptop with an Intel i7 2.8 GHz CPU and one Nvidia Quadro M2200 GPU. The FPS variation is due to the speed difference between the template matching submodule and the tracking submodule. 
Related results are reported in~\cref{sec:Preprocessing_exp}.

\subsection{Discussion}
There are a few points worthy of discussion:
\begin{itemize}
    \item Transfer learning could be employed to build the classifier based on some pre-trained networks if more lightweight and high-performance networks are available. Unfortunately, we did not find a suitable pre-trained network that can run in real-time on our laptop with a mid-range GPU. Most of the available pre-trained networks are too slow. For example, the famous pre-trained model VGG16 proposed by~\cite{simonyan2014very} took 0.5 seconds on our laptop to make an inference.
    \item There are a few state-of-the-arts object detectors like YoLo~\cite{redmon2016you} and Faster RCNN~\cite{ren2016faster} that can solve the object detection tasks very well. However, they rely on high-performance GPU. In case that the computational resource is limited, their efficiency will drop significantly. For instance, retrained Faster RCNN with a tiny classifier still takes around 0.15 s to process one frame on our laptop. Therefore, it is not worthwhile to integrate these methods into the fiducial detection module on our current computing platform. Nonetheless, they are still worthy of consideration if the computing platform can be upgraded.
\end{itemize}

